Noise Based Detection and Segmentation of Nebulous Objects

A noise-based non-parametric technique for detecting nebulous objects, for example, irregular or clumpy galaxies, and their structure in noise is introduced. "Noise-based" and "non-parametric" imply that this technique imposes negligible constraints on the properties of the targets and that it employs no regression analysis or fittings. The sub-sky detection threshold is defined and initial detections are found, independently of the sky value. False detections are then estimated and removed using the ambient noise as a reference. This results in a purity level of 0.89 for the final detections as compared to 0.29 for SExtractor when a completeness of 1 is desired for a sample of extremely faint and diffuse mock galaxy profiles. The difference in the mean of the undetected pixels with the known background of mock images is decreased by 4.6 times depending on the diffuseness of the test profiles, quantifying the success in their detection. A non-parametric approach to defining substructure over a detected region is also introduced. NoiseChisel is our software implementation of this new technique. Contrary to the existing signal-based approach to detection, in its various implementations, signal-related parameters such as the image point spread function or known object shapes and models are irrelevant here. Such features make this technique very useful in astrophysical applications such as detection, photometry, or morphological analysis of nebulous objects buried in noise, for example, galaxies that do not generically have a known shape when imaged.

==> Makefile <==
# Run LaTeX and BibLaTeX on a Tex source file. It is assumed that all
# the TeX source files are in a ./tex/ directory and the main .tex
# file is called paper.tex.
#
#
# TECHNICAL NOTE:
#
# If we simply use `$?' to check the return value, then it will be
# read from the make script and not within the shell script that is
# run within make. So we have to escape the $ sign with $$.

BIBname=./tex/ref.tex

paper.pdf: paper.tex tex/* paper.bbl reproduce/
#	rm -f ./tikz/paper-figure22.*
	mkdir -p tikz
	if [ -f paper.aux ]; then                                    \
	   if latex -shell-escape -halt-on-error paper.tex; then     \
	     echo "DVI made.";                                       \
	   else                                                      \
	     rm paper.aux;                                           \
	     exit 1;                                                 \
	   fi;                                                       \
	else                                                         \
	   if latex -shell-escape -halt-on-error paper.tex; then     \
	     echo "DVI made.";                                       \
	   else                                                      \
	     rm paper.aux;                                           \
	     exit 1;                                                 \
	   fi;                                                       \
	   latex -shell-escape paper.tex;                            \
	fi
	dvips -Ppdf paper.dvi
	ps2pdf paper.ps
#	rm paper.dvi
#	rm paper.ps
	if [ -f paper.blg ]; then rm paper.blg; fi
	if [ -f paper.run.xml ]; then rm paper.run.xml; fi
	if [ -f paper.auxlock ]; then rm paper.auxlock; fi
	rm paper.bcf paper.log paper.out

paper.bbl: $(BIBname)
	mkdir -p ./tikz/
	if latex -shell-escape -halt-on-error paper.tex; then        \
	  echo "DVI made.";                                          \
	else                                                         \
	  rm paper.aux;                                              \
	  exit 1;                                                    \
	fi;
	biber paper.bcf
	latex -shell-escape paper.tex;


==> reproduce/Makefile <==
# Reproduction Makefile for Akhlaghi et al. 2015:
#
# Title:      Noise based detection and segmentation of nebulous objects
# Author(s):  Mohammad Akhlaghi and Takashi Ichikawa
# Journal:    Astrophysical Journal Supplement Series
# doi:        10.1088/0067-0049/220/1/1
# arXiv:      1505.01664
# Year:       2015
# Volume:     220
# Article #:  1
#
# Copyright (C) 2015, Mohammad Akhlaghi <akhlaghi@astr.tohoku.ac.jp>
#
# This Makefile is free software: you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation, either version 3 of the License, or
# (at your option) any later version.
#
# This Makefile is distributed in the hope that it will be useful, but
# WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU
# General Public License for more details. See
# <http://www.gnu.org/licenses/>.
#
#
# If you are not familiar with the Makefile syntax, the comments
# (lines starting with a `#' sign) should be enough to understand
# everything about what each line does. An excellent resource for
# learning the Makefile syntax is the GNU Make manual (GNU Make is the
# most common implementation). It has wonderfully and completely
# explained all the concepts. It is available in various
# online/offline or print/digital formats at:
#
#     http://www.gnu.org/software/make/manual/










###################################################################
################       Basic preparations        ##################
###################################################################


# Outside directories
# ===================
#
# These directories are used outside of this Makefile and all its
# scripts. So please make sure you have made the proper changes
# outside this script if you want to change their values.

# The scripts that keep the instructioins:
export scripts=scripts/

# Input parameters for software and scripts.
export parameters=parameters/

# Read by LaTeX for important values.
export texmacro=texmacros.tex

# Images shipped with the code:
export images=$(parameters)/real/





# Internal variables
# ==================
export sexversion=2.19.5
gnuastro=$(parameters)/gnuastro/ast







# Read settings.mk
# ================
#
# All the parameters that are to be set by the user are stored and
# fully explained in the `settings.mk' file which is also in this
# directory. Here, that file is read and the variableS are exported to
# be availabe to all the scripts of this reproduction procedure.
include $(parameters)/reproduce/settings.mk
export CUTOUTS COSMOSACS SCCCD TMPDIR





# Internal directories
# ====================
#
# These directories keep the results of each step. Their names are
# chosen to be the same as the script and variable names for clarity.
export mock=$(TMPDIR)/mock/
export real=$(TMPDIR)/real/
export texdir=$(TMPDIR)/tex/
export catalog=$(TMPDIR)/catalog/
export mockparams=$(TMPDIR)/mockparams/
export sextractor=$(TMPDIR)/sextractor/
export noisechisel=$(TMPDIR)/noisechisel/
export scccdname=$(basename $(notdir $(SCCCD)))





# Internal files
# ==============
#
export realpsf=$(parameters)/sextractor/realpsf.conv
export realpositions=$(parameters)/real/realpositions.txt





# Target names
# ============
#
# These are the names of one of the files created by each script. It
# is best that the file be one of the last files created by the script
# so if the script has an error in the middle, it will be re-made the
# next time.
#
# These targets are needed in multiple steps during this make file:
#
#   1) To specify targets.
#   2) To specify prerequisits.
#
# So we have set variables for them to make the job easier, cleaner
# and remove the potential for bugs.
real_t=$(real)/6.fits
gnuastro_t=./.gnuastro/
papernumbers_t=$(texmacro)
mock_t=$(mock)/onelarge.fits
mockcat_t=$(mockparams)/purity.txt
sextractor_t=$(sextractor)/purity1.txt
paperfigures_t=$(texdir)/mode/mode2_stats.txt
noisechisel_t=$(noisechisel)/$(scccdname)_maskdet.fits



















###################################################################
################         Operation Rules         ##################
###################################################################
# This has to be the FIRST OPERATION. Define all the targets that
# should be created. The order of the rules is specified internally by
# Make depending on the dependencies. But we have tried to place the
# rules in the proper order below.
#all: $(gnuastro_t) $(mockcat_t) $(mock_t) $(real_t) $(noisechisel_t) \
#     $(sextractor_t) $(paperfigures_t) $(papernumbers_t)
all: $(gnuastro_t) $(mockcat_t) $(mock_t) $(paperfigures_t) $(papernumbers_t)





# Identify the phony targets (targets that are not actually a file) so
# Make doesn't look for a file with these names.
.PHONY: all clean distclean






# Make the current directory configuration file:
$(gnuastro_t):
	ln -s $(parameters)/gnuastro/ .gnuastro





# Make the catalogs (profile properties) for the mock images. Note
# that since there is no specific input we just echo a space to feed
# into AWK for it to start running the script.
$(mockcat_t): $(scripts)/mockcat.awk $(parameters)/reproduce/settings.awk
	mkdir -p $(mockparams)
	echo " " | awk -v outdir=$(mockparams) -i			\
	$(parameters)/reproduce/settings.awk -i $(scripts)/checks.awk	\
	-f scripts/mockcat.awk






# Make all the mock images necessary for this reproduction
$(mock_t): scripts/mock.sh $(mockcat_t) $(gnuastro)mkprof.conf          \
           $(gnuastro)convolve.conf $(gnuastro)imgwarp.conf             \
           $(gnuastro)mknoise.conf $(gnuastro)imgstat.conf
	./scripts/mock.sh





# Prepare the real images:
$(real_t): scripts/real.sh $(realpositions) $(gnuastro)imgcrop.conf
	./scripts/real.sh





# Run NoiseChisel:
$(noisechisel_t): scripts/noisechisel.sh $(real_t) $(mock_t)           \
                  $(gnuastro)noisechisel.conf $(gnuastro)mkcatalog.conf
	./scripts/noisechisel.sh





# Run SExtractor
$(sextractor_t): scripts/sextractor.sh $(real_t) $(mock_t)             \
                 $(parameters)/sextractor/sextractor.conf              \
                 $(parameters)/sextractor/sextractor.param 	       \
                 $(parameters)/sextractor/realpsf.conv
	./scripts/sextractor.sh





# Prepare the LaTeX/PGFPlots inputs
$(paperfigures_t): $(scripts)/paperfigures.sh $(scripts)/puritytf.awk  \
                   $(noisechisel_t) $(sextractor_t)                    \
                   $(gnuastro)mknoise.conf $(gnuastro)convertt.conf    \
                   $(gnuastro)imgcrop.conf $(gnuastro)imgstat.conf     \
                   $(gnuastro)convolve.conf $(gnuastro)imgwarp.conf    \
                   $(gnuastro)mkprof.conf
	./scripts/paperfigures.sh





# Prepare the numbers in the paper
$(papernumbers_t): $(scripts)/papernumbers.sh $(scripts)/puritytf.awk \
                   $(paperfigures_t) $(gnuastro)mkprof.conf           \
                   $(gnuastro)mknoise.conf $(gnuastro)noisechisel.conf\
                   $(gnuastro)imgstat.conf $(gnuastro)header.conf     \
                   $(parameters)/sextractor/sextractor.conf
	./scripts/papernumbers.sh




# Clean the working directory such that TeX can make all the figures,
# but all extra files are removed.
clean:
	rm -rf $(TMPDIR) *.log *.txt *.fits





# Clean everything
distclean:
	rm -rf $(TMPDIR) *.log *.txt *.fits $(texdir)


==> reproduce/README <==
Introduction
############

The contents of this directory provide the basic information (scripts
and parameter files) for the free quantitative reproduction of the
paper below.

Title:      Noise based detection and segmentation of nebulous objects
Author(s):  Mohammad Akhlaghi and Takashi Ichikawa
Journal:    Astrophysical Journal Supplement Series
doi:        10.1088/0067-0049/220/1/1
ADS code:   2015ApJS..220....1A
arXiv:      1505.01664
Year:       2015
Volume:     220
Article #:  1

"Free quantitative reproduction" is defined to be the fact that all
the numbers and plots of the paper can be exactly reproduced through
the scripts in this `reproduce' directory. All the software used are
"free" software enabling any curious scientist to easily check and
experiment on the source code of the software producing the
results. Nature is already a black box which we are trying hard to
understand. Not letting other scientists see the source code, or not
allowing them to modify it (do experiments on it) is a self-imposed
black box, which only exacerbates our ignorance.

Other scientists should be able to readily reproduce or check the
results of anything that is to carry the "scientific" adjective. Any
result that is not reproducible (due to incomplete information by the
author) is not scientific. Because the authors of those results expect
the readers to trust their result on faith in their subjective
experience.

See below on instructions on how to set the parameters of the
reproduction and the software requirements. With these two configured,
running the reproduction is as simple as running a `make'
command.

This is the first attempt at such a reproduction system (known by us),
so there might be unforeseen problems. Also, once a paper is submitted
to arXiv, it cannot be changed. Therefore, if there are any problems,
please visit the following address which is dedicated to the
reproduction of this paper:

http://astr.tohoku.ac.jp/~akhlaghi/reproduce/1505.01664/

If the issue has not been listed there, please contact
akhlaghi@astr.tohoku.ac.jp or akhlaghi@gnu.org.










Practical benefits
##################

Reproducability is the core basis of the proposed method. However, a
reproduction system like this also has lots of practical benefits. For
the actual researchers who are doing the research, this methodology is
very beneficial in the following aspects if it is adhered to from the
beginning:

 - Other team members in a research project can easily
   run/check/understand all the steps written by other members and
   find possibly better ways of reaching the result or implement
   their part of the research in a better fashion.

 - During the research project, it might happen that one of the
   parameters is decided to be changed or a new version of one of some
   of the software is released. With this system, updating all the
   numbers and plots in the paper is as simple as running a `make'
   command and the authors don't have to worry about part of the paper
   having the old configuration and the other part with the new
   configuration. Manually trying to change everything in the text
   will be prone to errors.

 - If the referee asks for another set of parameters, they can be
   immediately replaced and all the plots and numbers in the paper
   will be correspondingly updated.

 - Enabling version control on the contents of this reproduce
   directory will make reverting back to a previous state extremely
   simple, this is one of the main reasons the output TMPDIR directory
   is set to be another directory (see "Setting parameters" below). In
   this manner, only the source files which create the outputs are in
   this directory making version control very easy.

 - The authors are given the right to forget the details and keep
   their mind open. In any situation they can simply refer back to
   these scripts and see exactly what they did. This will enable
   researchers to be more open to learning/trying new methods without
   worrying about loosing/forgetting the details of their previous
   work. Since the contents of this `reproduce' directory are
   inherently very small, they can easily be uploaded on arXiv or
   other publication services.

For the community of the readers of the paper, this system has the
following advantages:

 - Other scientists can modify the parameters or the steps in order to
   check the effect of those changes on the plots and reported numbers
   and possibly find enhancements/problems in the result.

 - It serves as an excellent repository for students, or scientists
   with different specialties to master the art of data processing and
   analysis in this particular sub-field. By removing this barrier, it
   will enable the mixture of the experiences of the different fields,
   potentially leading to new insights and thus discoveries.

 - By changing the basic input parameters, the readers can try the
   exact same steps on other data-sets and check the result.

Of course, for all the situations above to be maximally effective, the
scripts have to be nicely commented.










How to reproduce
################

If the requirements are satisfied (see below), you can completely
reproduce the results with the following command within this directory
(you don't need to type the `$' sign):

    $ make

(Please read the Makefile for a complete explanation of the different
steps. If you are not familiar with the Makefile language, the
comments should be sufficient.)

Once it is complete, go up to the paper's LaTeX source directory which
was downloaded from arXiv. Open `paper.tex' and uncomment (remove the
`%' sign before) the line containing `\newcommand*{\makeeps}{}' which
is in the few top lines. This only needs to be done the first time you
get the source from arXiv. Then run `make again'. In short:

    $ cd ..
    $ gedit paper.tex
    $ make






Setting parameters
##################

All the major file and directory variables are within the
`parameters/reproduce/settings.mk' file. The comments above each
variable in that file explain the effect of that variable on the
script.

The major mock parameters can be set within the
`parameters/reproduce/settings.awk' file. These parameters are read by
the script which generates the mock catalogs which are then turned
into images and processed by other programs. Having read the paper,
the comments of each variable should be indicative enough of what they
do.


Updating figures
~~~~~~~~~~~~~~~~

The plots are made with the PGFPlots package within LaTeX. If
the figures are already present with a `tikz/' directory (which is
automatically made) and the source files have not changed, the same
figures will be used for the next LaTeX compilation. So if you have
already run the reproduction system once and decide to check how a
change of parameters would affect the figures, then remove the `tikz/'
directory before running Make in the top paper directory.

   $ rm -rf ./tikz/

If you only want to check the numbers, this is not needed. Also if you
already know the figure you want to check, then in order to speed up
the process, you can only delete the TikZ files related to that
figure. For example if only Figure 1 is desired, then run:

  $ rm ./tikz/paper-figure0.*


Last column of Figure 10
~~~~~~~~~~~~~~~~~~~~~~~~

The color codings of the images of the last column of Figure 10 are
specifically defined for NoiseChisel with the published set of input
parameters. If you are using different parameters, they will become
black. Please set the numbers by hand in `scripts/paperfigures.sh' as
explained in the comments above the part of this script for Figure 10.










Requirements
############

Software
~~~~~~~~

To reproduce the results you will need the following programs, other
versions might give different results.

The version of Gnuastro that was used to produce this paper is a
pre-release version labeled 0.0. It is available from the official
Gnuastro download link on its webpage. Gnuastro is still young and
under heavy development, so more recent versions might not produce
identical output.

lscpu is used to report the CPU frequency as reported in the
discussion section of the paper in `scripts/papernumbers.sh'.

Full program name         Short name     Version
------------------------------------------------------
GNU Astronomy Utilities   Gnuastro       0.0
Source Extractor          SExtractor     2.19.5
AWK                       AWK            any
lscpu                     Ships with the Linux kernel.

Data
~~~~

COSMOS galaxies:
----------------

The real galaxy images in this paper are from the COSMOS HST/ACS
images. If the science image tiles are available on your system or as a
local network address which you can access on the command-line like a
regular file, set the address of the directory containing the FITS
images as the value of the COSMOSACS variable in `settings.mk'.

The full archive of image tiles over this very wide field can be
downloaded from this address (only the Science images are necessary).

    http://irsa.ipac.caltech.edu/data/COSMOS/images/acs_mosaic_2.0/tiles/

The science images of all the tiles are roughly 136 Gigabytes! So if
you don't already have them, and you only want to reproduce the
results of this paper, it is easier to follow the alternative path
below.

Alternatively, you can get crops from the cutout tool at the survey
webpage. The coordinates of the real galaxies used are listed in the
following file:

    parameters/real/positions.txt

This file is formatted in the ASCII `IPAC table' format which you can
feed into the online cutout tool for the COSMOS survey. Set the size
of the images to 30 arcseconds = 1000 pixels and choose the "HST-ACS
Mosaic" in the "COSMOS Data Sets" table.

    http://irsa.ipac.caltech.edu/data/COSMOS/index_cutouts.html

There are multiple options once the download is complete, please
follow which ever method you like (the wget command is the easiest!
Just run the displayed command the directory you want the image to be
in and the FITS images will be put there). The outputs are ordered in
the same order of the table, so simply rename them to 1.fits, 2.fits,
until 6.fits. Then set the directory which keeps these fits images as
the value of the CUTOUTS variable in `settings.mk'.

Suprime-cam image:
------------------

Figure 11 uses one full CCD image recorded by Subaru Surpime-cam.
This image can be downloaded from the following URL:

    http://astr.tohoku.ac.jp/~akhlaghi/reproduce/1505.01664/CORR01269690.fits

Once you have downloaded it where ever you like, put its full file name
as the value of the SCCCD variable in `settings.mk'.










Contents
########

Before the reproduction, in this top `reproduce\' directory, there are
two directories and several files. The two files settings.mk and
settings.awk are used for setting the reproduction parameters. The
former is for setting the file and directory names and the latter for
the parameters of the most of the mock images in this paper. Both are
thoroughly commented for easy understanding of the significance of each
variable. The directory names are descriptive enough. The directories
are explained below:


parameters/
~~~~~~~~~~~

As the name suggests, this directory keeps all the parameters
necessary to create the mock and real input images, the parameters
necessary for SExtractor and the GNU Astronomy Utilities and also the
parameters to run this reproduction system. You can modify them and
see their effect on the produced paper.


scripts/
~~~~~~~~

The shell scripts in the `scripts' directory are the main work horse
of this reproduction system. They are called by the Makefile when
needed, their names are very descriptive. To see the order in which
they are run, please see the Makefile. If you search `.sh' in the
Makefile from the top of the file, you can see the scripts in the
order they are called. The make file is heavily commented, so you
don't necessarily have to know the Makefile syntax to understand what
is going on.










Acknowledgments
===============

Alan Lefor kindly helped in testing this reproduction system and we
are most grateful to him.

==> tex/ref.tex <==
%% This should actually have been ref.bib, but arXiv removes all files
%% ending with bib automatically. So it is named as ref.tex.



@ARTICLE{SDSSdeblender,
   author = {{Lupton}, R.~H.},
     year = 2015,
    month = aug,
    title = "{SDSS image processing I: the deblender}",
  journal = "{Personal home page}",
}





@ARTICLE{vanDokkum14,
   author = {{van Dokkum}, P.~G. and {Abraham}, R. and {Merritt}, A. and
	{Zhang}, J. and {Geha}, M. and {Conroy}, C.},
    title = "{Forty-seven Milky Way-sized, Extremely Diffuse Galaxies in the Coma Cluster}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1410.8141},
 keywords = {galaxies: clusters: individual: Coma, galaxies: evolution, galaxies: structure},
     year = 2015,
    month = jan,
   volume = 798,
    pages = {45},
      doi = {10.1088/2041-8205/798/2/L45},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798L..45V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@article{huang14,
 author = {Huang, Hao and Qin, Hong and Yoo, Shinjae and Yu, Dantong},
 title = {Physics-Based Anomaly Detection Defined on Manifold Space},
 journal = {ACM Trans. Knowl. Discov. Data},
 issue_date = {November 2014},
 volume = {9},
 number = {2},
 month = sep,
 year = {2014},
 issn = {1556-4681},
 pages = {14:1},
 articleno = {14},
 numpages = {39},
 url = {http://doi.acm.org/10.1145/2641574},
 doi = {10.1145/2641574},
 acmid = {2641574},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Anomaly detection, Laplace operator, heat diffusion, quantum mechanics},
}





@ARTICLE{abrahamvandokkum,
   author = {{Abraham}, R.~G. and {van Dokkum}, P.~G.},
    title = "{Ultra--Low Surface Brightness Imaging with the Dragonfly Telephoto Array}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1401.5473},
 primaryClass = "astro-ph.IM",
 keywords = {Astronomical Instrumentation},
     year = 2014,
    month = jan,
   volume = 126,
    pages = {55},
      doi = {10.1086/674875},
   adsurl = {http://adsabs.harvard.edu/abs/2014PASP..126...55A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{conselice14,
   author = {{Conselice}, C.~J.},
    title = "{The Evolution of Galaxy Structure Over Cosmic Time}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1403.2783},
     year = 2014,
    month = aug,
   volume = 52,
    pages = {291},
      doi = {10.1146/annurev-astro-081913-040037},
   adsurl = {http://adsabs.harvard.edu/abs/2014ARA&A..52..291C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{stripe822014,
   author = {{Jiang}, L. and {Fan}, X. and {Bian}, F. and {McGreer}, I.~D. and
	{Strauss}, M.~A. and {Annis}, J. and {Buck}, Z. and {Green}, R. and
	{Hodge}, J.~A. and {Myers}, A.~D. and {Rafiee}, A. and {Richards}, G.
	},
    title = "{The Sloan Digital Sky Survey Stripe 82 Imaging Data:
                  Depth-optimized Co-adds over 300 deg$^2$ in Five
                  Filters}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1405.7382},
 keywords = {atlases, catalogs, surveys },
     year = 2014,
    month = jul,
   volume = 213,
      eid = {12},
    pages = {12},
      doi = {10.1088/0067-0049/213/1/12},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJS..213...12J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{intraclusterlight,
   author = {{Presotto}, V. and {Girardi}, M. and {Nonino}, M. and {Mercurio}, A. and
	{Grillo}, C. and {Rosati}, P. and {Biviano}, A. and {Annunziatella}, M. and
	{Balestra}, I. and {Cui}, W. and {Sartoris}, B. and {Lemze}, D. and
	{Ascaso}, B. and {Moustakas}, J. and {Ford}, H. and {Fritz}, A. and
	{Czoske}, O. and {Ettori}, S. and {Kuchner}, U. and {Lombardi}, M. and
	{Maier}, C. and {Medezinski}, E. and {Molino}, A. and {Scodeggio}, M. and
	{Strazzullo}, V. and {Tozzi}, P. and {Ziegler}, B. and {Bartelmann}, M. and
	{Benitez}, N. and {Bradley}, L. and {Brescia}, M. and {Broadhurst}, T. and
	{Coe}, D. and {Donahue}, M. and {Gobat}, R. and {Graves}, G. and
	{Kelson}, D. and {Koekemoer}, A. and {Melchior}, P. and {Meneghetti}, M. and
	{Merten}, J. and {Moustakas}, L.~A. and {Munari}, E. and {Postman}, M. and
	{Reg{\H o}s}, E. and {Seitz}, S. and {Umetsu}, K. and {Zheng}, W. and
	{Zitrin}, A.},
    title = "{Intracluster light properties in the CLASH-VLT cluster MACS J1206.2-0847}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1403.4979},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: clusters: individual: MACS J1206.2-0847, cosmology: observations},
     year = 2014,
    month = may,
   volume = 565,
      eid = {A126},
    pages = {126},
      doi = {10.1051/0004-6361/201323251},
   adsurl = {http://adsabs.harvard.edu/abs/2014A&A...565A.126P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{skelton14,
   author = {{Skelton}, R.~E. and {Whitaker}, K.~E. and {Momcheva}, I.~G. and
	{Brammer}, G.~B. and {van Dokkum}, P.~G. and {Labb{\'e}}, I. and
	{Franx}, M. and {van der Wel}, A. and {Bezanson}, R. and {Da Cunha}, E. and
	{Fumagalli}, M. and {F{\"o}rster Schreiber}, N. and {Kriek}, M. and
	{Leja}, J. and {Lundgren}, B.~F. and {Magee}, D. and {Marchesini}, D. and
	{Maseda}, M.~V. and {Nelson}, E.~J. and {Oesch}, P. and {Pacifici}, C. and
	{Patel}, S.~G. and {Price}, S. and {Rix}, H.-W. and {Tal}, T. and
	{Wake}, D.~A. and {Wuyts}, S.},
    title = "{3D-HST WFC3-selected Photometric Catalogs in the Five CANDELS/3D-HST Fields: Photometry, Photometric Redshifts, and Stellar Masses}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1403.3689},
 keywords = {catalogs, galaxies: evolution, galaxies: general, methods: data analysis, techniques: photometric},
     year = 2014,
    month = oct,
   volume = 214,
      eid = {24},
    pages = {24},
      doi = {10.1088/0067-0049/214/2/24},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJS..214...24S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Murata14,
   author = {{Murata}, K.~L. and {Kajisawa}, M. and {Taniguchi}, Y. and {Kobayashi}, M.~A.~R. and
	{Shioya}, Y. and {Capak}, P. and {Ilbert}, O. and {Koekemoer}, A.~M. and
	{Salvato}, M. and {Scoville}, N.~Z.},
    title = "{Evolution of the Fraction of Clumpy Galaxies at 0.2 {\lt} z {\lt} 1.0 in the COSMOS Field}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1403.1496},
 keywords = {galaxies: evolution, galaxies: irregular, galaxies: star formation},
     year = 2014,
    month = may,
   volume = 786,
      eid = {15},
    pages = {15},
      doi = {10.1088/0004-637X/786/1/15},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...786...15M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{lundgren14,
   author = {{Lundgren}, B.~F. and {van Dokkum}, P. and {Franx}, M. and {Labbe}, I. and
	{Trenti}, M. and {Bouwens}, R. and {Gonzalez}, V. and {Illingworth}, G. and
	{Magee}, D. and {Oesch}, P. and {Stiavelli}, M.},
    title = "{Tracing the Mass Growth and Star Formation Rate Evolution of Massive Galaxies from z \~{} 6 to z \~{} 1 in the Hubble Ultra-Deep Field}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1310.7582},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: high-redshift, galaxies: stellar content},
     year = 2014,
    month = jan,
   volume = 780,
      eid = {34},
    pages = {34},
      doi = {10.1088/0004-637X/780/1/34},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...780...34L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{ellison13,
   author = {{Ellison}, S.~L. and {Mendel}, J.~T. and {Patton}, D.~R. and
	{Scudder}, J.~M.},
    title = "{Galaxy pairs in the Sloan Digital Sky Survey - VIII. The observational properties of post-merger galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1308.3707},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: abundances, galaxies: active, galaxies: evolution, galaxies: interactions, galaxies: Seyfert, galaxies: starburst},
     year = 2013,
    month = nov,
   volume = 435,
    pages = {3627},
      doi = {10.1093/mnras/stt1562},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.435.3627E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{XDFsurvey,
   author = {{Illingworth}, G.~D. and {Magee}, D. and {Oesch}, P.~A. and
	{Bouwens}, R.~J. and {Labb{\'e}}, I. and {Stiavelli}, M. and
	{van Dokkum}, P.~G. and {Franx}, M. and {Trenti}, M. and {Carollo}, C.~M. and
	{Gonzalez}, V.},
    title = "{The HST eXtreme Deep Field (XDF): Combining All ACS and WFC3/IR Data on the HUDF Region into the Deepest Field Ever}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1305.1931},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: observations, galaxies: abundances, galaxies: high-redshift, techniques: image processing },
     year = 2013,
    month = nov,
   volume = 209,
      eid = {6},
    pages = {6},
      doi = {10.1088/0067-0049/209/1/6},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..209....6I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{Lee2013,
   author = {{Lee}, B. and {Giavalisco}, M. and {Williams}, C.~C. and {Guo}, Y. and
	{Lotz}, J. and {Van der Wel}, A. and {Ferguson}, H.~C. and {Faber}, S.~M. and
	{Koekemoer}, A. and {Grogin}, N. and {Kocevski}, D. and {Conselice}, C.~J. and
	{Wuyts}, S. and {Dekel}, A. and {Kartaltepe}, J. and {Bell}, E.~F.
	},
    title = "{CANDELS: The Correlation between Galaxy Morphology and Star Formation Activity at z \~{} 2}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1306.4980},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: evolution, galaxies: formation, galaxies: high-redshift },
     year = 2013,
    month = sep,
   volume = 774,
      eid = {47},
    pages = {47},
      doi = {10.1088/0004-637X/774/1/47},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...774...47L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Mortlock13,
   author = {{Mortlock}, A. and {Conselice}, C.~J. and {Hartley}, W.~G. and
	{Ownsworth}, J.~R. and {Lani}, C. and {Bluck}, A.~F.~L. and
	{Almaini}, O. and {Duncan}, K. and {Wel}, A.~v.~d. and {Koekemoer}, A.~M. and
	{Dekel}, A. and {Dav{\'e}}, R. and {Ferguson}, H.~C. and {de Mello}, D.~F. and
	{Newman}, J.~A. and {Faber}, S.~M. and {Grogin}, N.~A. and {Kocevski}, D.~D. and
	{Lai}, K.},
    title = "{The redshift and mass dependence on the formation of the Hubble sequence at z {\gt} 1 from CANDELS/UDS}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1305.2204},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, galaxies: formation, galaxies: general, galaxies: structure},
     year = 2013,
    month = aug,
   volume = 433,
    pages = {1185},
      doi = {10.1093/mnras/stt793},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.433.1185M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{galametz2013,
   author = {{Galametz}, A. and {Grazian}, A. and {Fontana}, A. and {Ferguson}, H.~C. and
	{Ashby}, M.~L.~N. and {Barro}, G. and {Castellano}, M. and {Dahlen}, T. and
	{Donley}, J.~L. and {Faber}, S.~M. and {Grogin}, N. and {Guo}, Y. and
	{Huang}, K.-H. and {Kocevski}, D.~D. and {Koekemoer}, A.~M. and
	{Lee}, K.-S. and {McGrath}, E.~J. and {Peth}, M. and {Willner}, S.~P. and
	{Almaini}, O. and {Cooper}, M. and {Cooray}, A. and {Conselice}, C.~J. and
	{Dickinson}, M. and {Dunlop}, J.~S. and {Fazio}, G.~G. and {Foucaud}, S. and
	{Gardner}, J.~P. and {Giavalisco}, M. and {Hathi}, N.~P. and
	{Hartley}, W.~G. and {Koo}, D.~C. and {Lai}, K. and {de Mello}, D.~F. and
	{McLure}, R.~J. and {Lucas}, R.~A. and {Paris}, D. and {Pentericci}, L. and
	{Santini}, P. and {Simpson}, C. and {Sommariva}, V. and {Targett}, T. and
	{Weiner}, B.~J. and {Wuyts}, S. and {the CANDELS Team}},
    title = "{CANDELS Multiwavelength Catalogs: Source Identification and Photometry in the CANDELS UKIDSS Ultra-deep Survey Field}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1305.1823},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: photometry, methods: data analysis, techniques: image processing},
     year = 2013,
    month = jun,
   volume = 206,
      eid = {10},
    pages = {10},
      doi = {10.1088/0067-0049/206/2/10},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..206...10G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{muzzin13,
   author = {{Muzzin}, A. and {Marchesini}, D. and {Stefanon}, M. and {Franx}, M. and
	{Milvang-Jensen}, B. and {Dunlop}, J.~S. and {Fynbo}, J.~P.~U. and
	{Brammer}, G. and {Labb{\'e}}, I. and {van Dokkum}, P.},
    title = "{A Public K$_{s}$ -selected Catalog in the COSMOS/ULTRAVISTA Field: Photometry, Photometric Redshifts, and Stellar Population Parameters}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1303.4410},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, galaxies: fundamental parameters, galaxies: high-redshift, infrared: galaxies},
     year = 2013,
    month = may,
   volume = 206,
      eid = {8},
    pages = {8},
      doi = {10.1088/0067-0049/206/1/8},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..206....8M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{vollmer13,
   author = {{Vollmer}, B. and {Perret}, B. and {Petremand}, M. and {Lavigne}, F. and
	{Collet}, C. and {van Driel}, W. and {Bonnarel}, F. and {Louys}, M. and
	{Sabatini}, S. and {MacArthur}, L.~A.},
    title = "{Simultaneous Multi-band Detection of Low Surface Brightness Galaxies with Markovian Modeling}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1211.4687},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: clusters: individual: Virgo, galaxies: fundamental parameters, methods: data analysis, techniques: image processing},
     year = 2013,
    month = feb,
   volume = 145,
      eid = {36},
    pages = {36},
      doi = {10.1088/0004-6256/145/2/36},
   adsurl = {http://adsabs.harvard.edu/abs/2013AJ....145...36V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{vdWel12,
   author = {{van der Wel}, A. and {Bell}, E.~F. and {H{\"a}ussler}, B. and
	{McGrath}, E.~J. and {Chang}, Y.-Y. and {Guo}, Y. and {McIntosh}, D.~H. and
	{Rix}, H.-W. and {Barden}, M. and {Cheung}, E. and {Faber}, S.~M. and
	{Ferguson}, H.~C. and {Galametz}, A. and {Grogin}, N.~A. and
	{Hartley}, W. and {Kartaltepe}, J.~S. and {Kocevski}, D.~D. and
	{Koekemoer}, A.~M. and {Lotz}, J. and {Mozena}, M. and {Peth}, M.~A. and
	{Peng}, C.~Y.},
    title = "{Structural Parameters of Galaxies in CANDELS}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1211.6954},
 primaryClass = "astro-ph.CO",
 keywords = {catalogs, galaxies: high-redshift, galaxies: statistics, galaxies: structure, surveys },
     year = 2012,
    month = dec,
   volume = 203,
      eid = {24},
    pages = {24},
      doi = {10.1088/0067-0049/203/2/24},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJS..203...24V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{wuyts12,
   author = {{Wuyts}, S. and {F{\"o}rster Schreiber}, N.~M. and {Genzel}, R. and
	{Guo}, Y. and {Barro}, G. and {Bell}, E.~F. and {Dekel}, A. and
	{Faber}, S.~M. and {Ferguson}, H.~C. and {Giavalisco}, M. and
	{Grogin}, N.~A. and {Hathi}, N.~P. and {Huang}, K.-H. and {Kocevski}, D.~D. and
	{Koekemoer}, A.~M. and {Koo}, D.~C. and {Lotz}, J. and {Lutz}, D. and
	{McGrath}, E. and {Newman}, J.~A. and {Rosario}, D. and {Saintonge}, A. and
	{Tacconi}, L.~J. and {Weiner}, B.~J. and {van der Wel}, A.},
    title = "{Smooth(er) Stellar Mass Maps in CANDELS: Constraints on the Longevity of Clumps in High-redshift Star-forming Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1203.2611},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: high-redshift, galaxies: stellar content, galaxies: structure},
     year = 2012,
    month = jul,
   volume = 753,
      eid = {114},
    pages = {114},
      doi = {10.1088/0004-637X/753/2/114},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...753..114W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@BOOK{drizzlepac,
   author = {{Gonzaga}, S. and {Hack}, W. and {Fruchter}, A. and {Mack}, J.},
    title = "{The DrizzlePac Handbook}",
 keywords = {DrizzlePac, AstroDrizzle, TweakReg, dither, multidrizzle, drizzle, HST },
booktitle = {The DrizzlePac Handbook, HST Data Handbook},
     year = 2012,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2012drzp.book.....G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{galapagos,
   author = {{Barden}, M. and {H{\"a}u{\ss}ler}, B. and {Peng}, C.~Y. and
	{McIntosh}, D.~H. and {Guo}, Y.},
    title = "{GALAPAGOS: from pixels to parameters}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1203.1831},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, surveys, galaxies: statistics, galaxies: structure},
     year = 2012,
    month = may,
   volume = 422,
    pages = {449},
      doi = {10.1111/j.1365-2966.2012.20619.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422..449B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{lackner12,
   author = {{Lackner}, C.~N. and {Gunn}, J.~E.},
    title = "{Astrophysically motivated bulge-disc decompositions of Sloan Digital Sky Survey galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1201.0763},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: bulges, galaxies: evolution, galaxies: photometry, galaxies: structure},
     year = 2012,
    month = apr,
   volume = 421,
    pages = {2277},
      doi = {10.1111/j.1365-2966.2012.20450.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421.2277L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{stripe82,
   author = {{Annis}, J. and {Soares-Santos}, M. and {Strauss}, M.~A. and
	{Becker}, A.~C. and {Dodelson}, S. and {Fan}, X. and {Gunn}, J.~E. and
	{Hao}, J. and {Ivezi{\'c}}, {\v Z}. and {Jester}, S. and {Jiang}, L. and
	{Johnston}, D.~E. and {Kubo}, J.~M. and {Lampeitl}, H. and {Lin}, H. and
	{Lupton}, R.~H. and {Miknaitis}, G. and {Seo}, H.-J. and {Simet}, M. and
	{Yanny}, B.},
    title = "{The Sloan Digital Sky Survey Coadd: 275{\nbsp}deg$^{2}$ of Deep Sloan Digital Sky Survey Imaging on Stripe 82}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1111.6619},
 keywords = {atlases, catalogs, surveys },
     year = 2014,
    month = oct,
   volume = 794,
      eid = {120},
    pages = {120},
      doi = {10.1088/0004-637X/794/2/120},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...794..120A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{tinytim,
   author = {{Krist}, J.~E. and {Hook}, R.~N. and {Stoehr}, F.},
    title = "{20 years of Hubble Space Telescope optical modeling using Tiny Tim}",
  journal = {Proc. SPIE},
     year = 2011,
   volume = 8127,
    month = oct,
      eid = {81270J},
    pages = {0},
      doi = {10.1117/12.892762},
   adsurl = {http://adsabs.harvard.edu/abs/2011SPIE.8127E..0JK},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{sdssdr8,
   author = {{Aihara}, H. and {Allende Prieto}, C. and {An}, D. and {Anderson}, S.~F. and
	{Aubourg}, {\'E}. and {Balbinot}, E. and {Beers}, T.~C. and
	{Berlind}, A.~A. and {Bickerton}, S.~J. and {Bizyaev}, D. and
	{Blanton}, M.~R. and {Bochanski}, J.~J. and {Bolton}, A.~S. and
	{Bovy}, J. and {Brandt}, W.~N. and {Brinkmann}, J. and {Brown}, P.~J. and
	{Brownstein}, J.~R. and {Busca}, N.~G. and {Campbell}, H. and
	{Carr}, M.~A. and {Chen}, Y. and {Chiappini}, C. and {Comparat}, J. and
	{Connolly}, N. and {Cortes}, M. and {Croft}, R.~A.~C. and {Cuesta}, A.~J. and
	{da Costa}, L.~N. and {Davenport}, J.~R.~A. and {Dawson}, K. and
	{Dhital}, S. and {Ealet}, A. and {Ebelke}, G.~L. and {Edmondson}, E.~M. and
	{Eisenstein}, D.~J. and {Escoffier}, S. and {Esposito}, M. and
	{Evans}, M.~L. and {Fan}, X. and {Femen{\'{\i}}a Castell{\'a}}, B. and
	{Font-Ribera}, A. and {Frinchaboy}, P.~M. and {Ge}, J. and {Gillespie}, B.~A. and
	{Gilmore}, G. and {Gonz{\'a}lez Hern{\'a}ndez}, J.~I. and {Gott}, J.~R. and
	{Gould}, A. and {Grebel}, E.~K. and {Gunn}, J.~E. and {Hamilton}, J.-C. and
	{Harding}, P. and {Harris}, D.~W. and {Hawley}, S.~L. and {Hearty}, F.~R. and
	{Ho}, S. and {Hogg}, D.~W. and {Holtzman}, J.~A. and {Honscheid}, K. and
	{Inada}, N. and {Ivans}, I.~I. and {Jiang}, L. and {Johnson}, J.~A. and
	{Jordan}, C. and {Jordan}, W.~P. and {Kazin}, E.~A. and {Kirkby}, D. and
	{Klaene}, M.~A. and {Knapp}, G.~R. and {Kneib}, J.-P. and {Kochanek}, C.~S. and
	{Koesterke}, L. and {Kollmeier}, J.~A. and {Kron}, R.~G. and
	{Lampeitl}, H. and {Lang}, D. and {Le Goff}, J.-M. and {Lee}, Y.~S. and
	{Lin}, Y.-T. and {Long}, D.~C. and {Loomis}, C.~P. and {Lucatello}, S. and
	{Lundgren}, B. and {Lupton}, R.~H. and {Ma}, Z. and {MacDonald}, N. and
	{Mahadevan}, S. and {Maia}, M.~A.~G. and {Makler}, M. and {Malanushenko}, E. and
	{Malanushenko}, V. and {Mandelbaum}, R. and {Maraston}, C. and
	{Margala}, D. and {Masters}, K.~L. and {McBride}, C.~K. and
	{McGehee}, P.~M. and {McGreer}, I.~D. and {M{\'e}nard}, B. and
	{Miralda-Escud{\'e}}, J. and {Morrison}, H.~L. and {Mullally}, F. and
	{Muna}, D. and {Munn}, J.~A. and {Murayama}, H. and {Myers}, A.~D. and
	{Naugle}, T. and {Neto}, A.~F. and {Nguyen}, D.~C. and {Nichol}, R.~C. and
	{O'Connell}, R.~W. and {Ogando}, R.~L.~C. and {Olmstead}, M.~D. and
	{Oravetz}, D.~J. and {Padmanabhan}, N. and {Palanque-Delabrouille}, N. and
	{Pan}, K. and {Pandey}, P. and {P{\^a}ris}, I. and {Percival}, W.~J. and
	{Petitjean}, P. and {Pfaffenberger}, R. and {Pforr}, J. and
	{Phleps}, S. and {Pichon}, C. and {Pieri}, M.~M. and {Prada}, F. and
	{Price-Whelan}, A.~M. and {Raddick}, M.~J. and {Ramos}, B.~H.~F. and
	{Reyl{\'e}}, C. and {Rich}, J. and {Richards}, G.~T. and {Rix}, H.-W. and
	{Robin}, A.~C. and {Rocha-Pinto}, H.~J. and {Rockosi}, C.~M. and
	{Roe}, N.~A. and {Rollinde}, E. and {Ross}, A.~J. and {Ross}, N.~P. and
	{Rossetto}, B.~M. and {S{\'a}nchez}, A.~G. and {Sayres}, C. and
	{Schlegel}, D.~J. and {Schlesinger}, K.~J. and {Schmidt}, S.~J. and
	{Schneider}, D.~P. and {Sheldon}, E. and {Shu}, Y. and {Simmerer}, J. and
	{Simmons}, A.~E. and {Sivarani}, T. and {Snedden}, S.~A. and
	{Sobeck}, J.~S. and {Steinmetz}, M. and {Strauss}, M.~A. and
	{Szalay}, A.~S. and {Tanaka}, M. and {Thakar}, A.~R. and {Thomas}, D. and
	{Tinker}, J.~L. and {Tofflemire}, B.~M. and {Tojeiro}, R. and
	{Tremonti}, C.~A. and {Vandenberg}, J. and {Vargas Maga{\~n}a}, M. and
	{Verde}, L. and {Vogt}, N.~P. and {Wake}, D.~A. and {Wang}, J. and
	{Weaver}, B.~A. and {Weinberg}, D.~H. and {White}, M. and {White}, S.~D.~M. and
	{Yanny}, B. and {Yasuda}, N. and {Yeche}, C. and {Zehavi}, I.
	},
    title = "{The Eighth Data Release of the Sloan Digital Sky Survey: First Data from SDSS-III}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1101.1559},
 primaryClass = "astro-ph.IM",
 keywords = {atlases, catalogs, surveys},
     year = 2011,
    month = apr,
   volume = 193,
      eid = {29},
    pages = {29},
      doi = {10.1088/0067-0049/193/2/29},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..193...29A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{kaj2011,
   author = {{Kajisawa}, M. and {Ichikawa}, T. and {Tanaka}, I. and {Yamada}, T. and
	{Akiyama}, M. and {Suzuki}, R. and {Tokoku}, C. and {Katsuno Uchimoto}, Y. and
	{Konishi}, M. and {Yoshikawa}, T. and {Nishimura}, T. and {Omata}, K. and
	{Ouchi}, M. and {Iwata}, I. and {Hamana}, T. and {Onodera}, M.
	},
    title = "{MOIRCS Deep Survey. IX. Deep Near-Infrared Imaging Data and Source Catalog}",
  journal = {\pasj},
archivePrefix = "arXiv",
   eprint = {1012.2115},
 keywords = {catalogs, galaxies: high-redshift, galaxies: photometry, infrared: galaxies, surveys},
     year = 2011,
    month = mar,
   volume = 63,
    pages = {379},
      doi = {10.1093/pasj/63.sp2.S379},
   adsurl = {http://adsabs.harvard.edu/abs/2011PASJ...63S.379K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{kaj2010,
   author = {{Kajisawa}, M. and {Ichikawa}, T. and {Yamada}, T. and {Uchimoto}, Y.~K. and
	{Yoshikawa}, T. and {Akiyama}, M. and {Onodera}, M.},
    title = "{MOIRCS Deep Survey. VIII. Evolution of Star Formation Activity as a Function of Stellar Mass in Galaxies Since z \~{} 3}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1009.0002},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, galaxies: high-redshift, infrared: galaxies},
     year = 2010,
    month = nov,
   volume = 723,
    pages = {129},
      doi = {10.1088/0004-637X/723/1/129},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...723..129K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{galfit,
   author = {{Peng}, C.~Y. and {Ho}, L.~C. and {Impey}, C.~D. and {Rix}, H.-W.
	},
    title = "{Detailed Decomposition of Galaxy Images. II. Beyond Axisymmetric Models}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0912.0731},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: bulges, galaxies: fundamental parameters, galaxies: structure, techniques: image processing, techniques: photometric},
     year = 2010,
    month = jun,
   volume = 139,
    pages = {2097},
      doi = {10.1088/0004-6256/139/6/2097},
   adsurl = {http://adsabs.harvard.edu/abs/2010AJ....139.2097P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{maccio2010,
   author = {{Macci{\`o}}, A.~V. and {Kang}, X. and {Fontanot}, F. and {Somerville}, R.~S. and
	{Koposov}, S. and {Monaco}, P.},
    title = "{Luminosity function and radial distribution of Milky Way satellites in a {$\Lambda$}CDM Universe}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0903.4681},
 primaryClass = "astro-ph.CO",
 keywords = {gravitation, methods: N-body simulation, methods: numerical, galaxies: haloes, cosmology: theory, dark matter},
     year = 2010,
    month = mar,
   volume = 402,
    pages = {1995},
      doi = {10.1111/j.1365-2966.2009.16031.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.402.1995M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{massy10,
   author = {{Massey}, R. and {Stoughton}, C. and {Leauthaud}, A. and {Rhodes}, J. and
	{Koekemoer}, A. and {Ellis}, R. and {Shaghoulian}, E.},
    title = "{Pixel-based correction for Charge Transfer Inefficiency in the Hubble Space Telescope Advanced Camera for Surveys}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0909.0507},
 keywords = {instrumentation: detectors, methods: data analysis, space vehicles: instruments},
     year = 2010,
    month = jan,
   volume = 401,
    pages = {371},
      doi = {10.1111/j.1365-2966.2009.15638.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.401..371M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@article{chandola09,
 author = {{Chandola}, V. and {Banerjee}, A. and {Kumar}, V.},
 title = {Anomaly Detection: A Survey},
 journal = {ACM Comput. Surv.},
 issue_date = {July 2009},
 volume = {41},
 number = {3},
 month = jul,
 year = {2009},
 issn = {0360-0300},
 pages = {15:1},
 articleno = {15},
 numpages = {58},
 url = {http://doi.acm.org/10.1145/1541880.1541882},
 doi = {10.1145/1541880.1541882},
 acmid = {1541882},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Anomaly detection, outlier detection},
}





@article{perret09,
 author = {{Perret}, B. and {Lef\'evre}, S. and {Collet}, Ch.},
 title = {A robust hit or miss transform for template matching applied to very noisy astronomical images},
 journal = {Pattern Recognition},
 doi = {10.1016/j.patcog.2009.02.013},
 volume = {42},
 year = {2009},
 pages = {2470},
}







@ARTICLE{kormendy09,
   author = {{Kormendy}, J. and {Fisher}, D.~B. and {Cornell}, M.~E. and
	{Bender}, R.},
    title = "{Structure and Formation of Elliptical and Spheroidal Galaxies}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {0810.1681},
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: nuclei, galaxies: photometry, galaxies: structure},
     year = 2009,
    month = may,
   volume = 182,
    pages = {216},
      doi = {10.1088/0067-0049/182/1/216},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJS..182..216K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@book{eimginastro,
    author    = "{McLean}, I. S.",
    title     = "Electronic imaging in astronomy",
    publisher = "Praxis Publishing Ltd",
    edition   = "2nd",
    year      = "2008",
    isbn      = "978-3-540-76582-0"
}





@book{gonzalezwoods,
 author    = "{Gonzalez}, R.~C. and {Woods}, R.E.",
 title     = "Digital Image Processing",
 publisher = "Prentice Hall",
 year      =  2008,
 edition   = "3rd",
 isbn      = "978-0131687288"
}





@ARTICLE{cosmos,
   author = {{Scoville}, N. and {Aussel}, H. and {Brusa}, M. and {Capak}, P. and
	{Carollo}, C.~M. and {Elvis}, M. and {Giavalisco}, M. and {Guzzo}, L. and
	{Hasinger}, G. and {Impey}, C. and {Kneib}, J.-P. and {LeFevre}, O. and
	{Lilly}, S.~J. and {Mobasher}, B. and {Renzini}, A. and {Rich}, R.~M. and
	{Sanders}, D.~B. and {Schinnerer}, E. and {Schminovich}, D. and
	{Shopbell}, P. and {Taniguchi}, Y. and {Tyson}, N.~D.},
    title = "{The Cosmic Evolution Survey (COSMOS): Overview}",
  journal = {\apjs},
   eprint = {astro-ph/0612305},
 keywords = {Cosmology: Observations, Cosmology: Dark Matter, Galaxies: Evolution, Galaxies: Formation, Cosmology: Large-Scale Structure of Universe, Surveys},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {1},
      doi = {10.1086/516585},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172....1S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{cosmoshstiband,
   author = {{Koekemoer}, A.~M. and {Aussel}, H. and {Calzetti}, D. and {Capak}, P. and
	{Giavalisco}, M. and {Kneib}, J.-P. and {Leauthaud}, A. and
	{Le F{\`e}vre}, O. and {McCracken}, H.~J. and {Massey}, R. and
	{Mobasher}, B. and {Rhodes}, J. and {Scoville}, N. and {Shopbell}, P.~L.
	},
    title = "{The COSMOS Survey: Hubble Space Telescope Advanced Camera for Surveys Observations and Data Processing}",
  journal = {\apjs},
   eprint = {astro-ph/0703095},
 keywords = {Cosmology: Observations, Cosmology: Dark Matter, Galaxies: Evolution, Galaxies: Formation, Cosmology: Large-Scale Structure of Universe, Surveys},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {196},
      doi = {10.1086/520086},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172..196K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{leuthaud07,
   author = {{Leauthaud}, A. and {Massey}, R. and {Kneib}, J.-P. and {Rhodes}, J. and
	{Johnston}, D.~E. and {Capak}, P. and {Heymans}, C. and {Ellis}, R.~S. and
	{Koekemoer}, A.~M. and {Le F{\`e}vre}, O. and {Mellier}, Y. and
	{R{\'e}fr{\'e}gier}, A. and {Robin}, A.~C. and {Scoville}, N. and
	{Tasca}, L. and {Taylor}, J.~E. and {Van Waerbeke}, L.},
    title = "{Weak Gravitational Lensing with COSMOS: Galaxy Selection and Shape Measurements}",
  journal = {\apjs},
   eprint = {astro-ph/0702359},
 keywords = {Cosmology: Observations, Cosmology: Gravitational Lensing, Cosmology: Large-Scale Structure of Universe},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {219},
      doi = {10.1086/516598},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172..219L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{lauer07,
   author = {{Lauer}, T.~R. and {Faber}, S.~M. and {Richstone}, D. and {Gebhardt}, K. and
	{Tremaine}, S. and {Postman}, M. and {Dressler}, A. and {Aller}, M.~C. and
	{Filippenko}, A.~V. and {Green}, R. and {Ho}, L.~C. and {Kormendy}, J. and
	{Magorrian}, J. and {Pinkney}, J.},
    title = "{The Masses of Nuclear Black Holes in Luminous Elliptical Galaxies and Implications for the Space Density of the Most Massive Black Holes}",
  journal = {\apj},
   eprint = {astro-ph/0606739},
 keywords = {Black Hole Physics, Galaxies: Nuclei, Galaxies: Structure},
     year = 2007,
    month = jun,
   volume = 662,
    pages = {808},
      doi = {10.1086/518223},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...662..808L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{elmegreen2007,
   author = {{Elmegreen}, D.~M. and {Elmegreen}, B.~G. and {Ravindranath}, S. and
	{Coe}, D.~A.},
    title = "{Resolved Galaxies in the Hubble Ultra Deep Field: Star Formation in Disks at High Redshift}",
  journal = {\apj},
   eprint = {astro-ph/0701121},
 keywords = {Galaxies: Evolution, Galaxies: Formation, Galaxies: High-Redshift},
     year = 2007,
    month = apr,
   volume = 658,
    pages = {763},
      doi = {10.1086/511667},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...658..763E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{hopkins06,
   author = {{Hopkins}, A.~M. and {Beacom}, J.~F.},
    title = "{On the Normalization of the Cosmic Star Formation History}",
  journal = {\apj},
   eprint = {astro-ph/0601463},
 keywords = {Galaxies: Evolution, Galaxies: Formation, Galaxies: Starburst, Neutrinos, Stars: Supernovae: General},
     year = 2006,
    month = nov,
   volume = 651,
    pages = {142},
      doi = {10.1086/506610},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...651..142H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{pohlen06,
   author = {{Pohlen}, M. and {Trujillo}, I.},
    title = "{The structure of galactic disks. Studying late-type spiral galaxies using SDSS}",
  journal = {\aap},
   eprint = {astro-ph/0603682},
 keywords = {galaxies: photometry, galaxies: structure, galaxies: fundamental parameters, galaxies: evolution, galaxies: formation},
     year = 2006,
    month = aug,
   volume = 454,
    pages = {759},
      doi = {10.1051/0004-6361:20064883},
   adsurl = {http://adsabs.harvard.edu/abs/2006A&A...454..759P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{lotz06,
   author = {{Lotz}, J.~M. and {Madau}, P. and {Giavalisco}, M. and {Primack}, J. and
	{Ferguson}, H.~C.},
    title = "{The Rest-Frame Far-Ultraviolet Morphologies of Star-forming Galaxies at z \~{} 1.5 and 4}",
  journal = {\apj},
 keywords = {Galaxies: Evolution, Galaxies: High-Redshift, Galaxies: Interactions, Galaxies: Structure, Ultraviolet: Galaxies},
     year = 2006,
    month = jan,
   volume = 636,
    pages = {592},
      doi = {10.1086/497950},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...636..592L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@book{starckmurtagh,
 author    = "{Starck}, J. and {Murtagh}, F.",
 title     = "Astronomical Image and Data Analysis",
 publisher = "Springer",
 year      =  2006,
 edition   = "2nd",
 isbn      = "978-3-662-04908-2"
}





@ARTICLE{grahamdriver05,
   author = {{Graham}, A.~W. and {Driver}, S.~P.},
    title = "{A Concise Reference to (Projected) S{\'e}rsic R$^{1/n}$ Quantities, Including Concentration, Profile Slopes, Petrosian Indices, and Kron Magnitudes}",
  journal = {\pasa},
   eprint = {astro-ph/0503176},
 keywords = {galaxies: structure, galaxies: fundamental parameters, methods: analytical, methods: data analysis},
     year = 2005,
   volume = 22,
    pages = {118},
      doi = {10.1071/AS05001},
   adsurl = {http://adsabs.harvard.edu/abs/2005PASA...22..118G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{cayon05,
   author = {{Cay{\'o}n}, L. and {Jin}, J. and {Treaster}, A.},
    title = "{Higher Criticism statistic: detecting and identifying non-Gaussianity in the WMAP first-year data}",
  journal = {\mnras},
   eprint = {astro-ph/0507246},
 keywords = {methods: statistical, cosmic microwave background, cosmology: miscellaneous},
     year = 2005,
    month = sep,
   volume = 362,
    pages = {826},
      doi = {10.1111/j.1365-2966.2005.09277.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.362..826C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{mandelbaum05,
   author = {{Mandelbaum}, R. and {Hirata}, C.~M. and {Seljak}, U. and {Guzik}, J. and
	{Padmanabhan}, N. and {Blake}, C. and {Blanton}, M.~R. and {Lupton}, R. and
	{Brinkmann}, J.},
    title = "{Systematic errors in weak lensing: application to SDSS galaxy-galaxy weak lensing}",
  journal = {\mnras},
   eprint = {astro-ph/0501201},
 keywords = {gravitational lensing, galaxies: distances and redshifts, galaxies: halos},
     year = 2005,
    month = aug,
   volume = 361,
    pages = {1287},
      doi = {10.1111/j.1365-2966.2005.09282.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.361.1287M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{kregel2004,
   author = {{Kregel}, M. and {van der Kruit}, P.~C.},
    title = "{Radial truncations in stellar discs in galaxies}",
  journal = {\mnras},
   eprint = {astro-ph/0408125},
 keywords = {galaxies: fundamental parameters, galaxies: spiral, galaxies: structure},
     year = 2004,
    month = nov,
   volume = 355,
    pages = {143},
      doi = {10.1111/j.1365-2966.2004.08307.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.355..143K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{rix04,
   author = {{Rix}, H.-W. and {Barden}, M. and {Beckwith}, S.~V.~W. and {Bell}, E.~F. and
	{Borch}, A. and {Caldwell}, J.~A.~R. and {H{\"a}ussler}, B. and
	{Jahnke}, K. and {Jogee}, S. and {McIntosh}, D.~H. and {Meisenheimer}, K. and
	{Peng}, C.~Y. and {Sanchez}, S.~F. and {Somerville}, R.~S. and
	{Wisotzki}, L. and {Wolf}, C.},
    title = "{GEMS: Galaxy Evolution from Morphologies and SEDs}",
  journal = {\apjs},
   eprint = {astro-ph/0401427},
 keywords = {Galaxies: Bulges, Galaxies: Evolution, Galaxies: Fundamental Parameters, Galaxies: High-Redshift, Galaxies: Structure},
     year = 2004,
    month = jun,
   volume = 152,
    pages = {163},
      doi = {10.1086/420885},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..152..163R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{highercriticism,
   author = {{Donoho}, D. and {Jin}, J.},
    title = "{Higher criticism for detecting sparse heterogeneous
                  mixtures}",
  journal = {The annals of Statistics},
     year = 2004,
   volume = 32,
    pages = {962},
      doi = {10.1214/009053604000000265},
}






@ARTICLE{Benitez04,
   author = {{Ben{\'{\i}}tez}, N. and {Ford}, H. and {Bouwens}, R. and {Menanteau}, F. and
	{Blakeslee}, J. and {Gronwall}, C. and {Illingworth}, G. and
	{Meurer}, G. and {Broadhurst}, T.~J. and {Clampin}, M. and {Franx}, M. and
	{Hartig}, G.~F. and {Magee}, D. and {Sirianni}, M. and {Ardila}, D.~R. and
	{Bartko}, F. and {Brown}, R.~A. and {Burrows}, C.~J. and {Cheng}, E.~S. and
	{Cross}, N.~J.~G. and {Feldman}, P.~D. and {Golimowski}, D.~A. and
	{Infante}, L. and {Kimble}, R.~A. and {Krist}, J.~E. and {Lesser}, M.~P. and
	{Levay}, Z. and {Martel}, A.~R. and {Miley}, G.~K. and {Postman}, M. and
	{Rosati}, P. and {Sparks}, W.~B. and {Tran}, H.~D. and {Tsvetanov}, Z.~I. and
	{White}, R.~L. and {Zheng}, W.},
    title = "{Faint Galaxies in Deep Advanced Camera for Surveys Observations}",
  journal = {\apjs},
 keywords = {Galaxies: Evolution, Galaxies: Fundamental Parameters, Galaxies: High-Redshift, Galaxies: Photometry, Techniques: Photometric},
     year = 2004,
    month = jan,
   volume = 150,
    pages = {1},
      doi = {10.1086/380120},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..150....1B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{suprimecam,
   author = {{Miyazaki}, S. and {Komiyama}, Y. and {Sekiguchi}, M. and {Okamura}, S. and
	{Doi}, M. and {Furusawa}, H. and {Hamabe}, M. and {Imi}, K. and
	{Kimura}, M. and {Nakata}, F. and {Okada}, N. and {Ouchi}, M. and
	{Shimasaku}, K. and {Yagi}, M. and {Yasuda}, N.},
    title = "{Subaru Prime Focus Camera -- Suprime-Cam}",
  journal = {\pasj},
   eprint = {astro-ph/0211006},
 keywords = {instrumentation: detectors, techniques: image processing, telescopes},
     year = 2002,
    month = dec,
   volume = 54,
    pages = {833},
      doi = {10.1093/pasj/54.6.833},
   adsurl = {http://adsabs.harvard.edu/abs/2002PASJ...54..833M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Bernstein02b,
   author = {{Bernstein}, R.~A. and {Freedman}, W.~L. and {Madore}, B.~F.
	},
    title = "{The First Detections of the Extragalactic Background Light at 3000, 5500, and 8000 {\AA}. III. Cosmological Implications}",
  journal = {\apj},
   eprint = {astro-ph/0112170},
 keywords = {Cosmology: Observations, Cosmology: Diffuse Radiation, Galaxies: Evolution, Galaxies: Photometry},
     year = 2002,
    month = may,
   volume = 571,
    pages = {107},
      doi = {10.1086/339424},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...571..107B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Bernstein02a,
   author = {{Bernstein}, R.~A. and {Freedman}, W.~L. and {Madore}, B.~F.
	},
    title = "{The First Detections of the Extragalactic Background Light at 3000, 5500, and 8000 {\AA}. I. Results}",
  journal = {\apj},
   eprint = {astro-ph/0112153},
 keywords = {Cosmology: Observations, Cosmology: Diffuse Radiation, ISM: Dust, Extinction- Galaxies: Photometry, Interplanetary Medium, Techniques: Photometric},
     year = 2002,
    month = may,
   volume = 571,
    pages = {56},
      doi = {10.1086/339422},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...571...56B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{hopkins02,
   author = {{Hopkins}, A.~M. and {Miller}, C.~J. and {Connolly}, A.~J. and
	{Genovese}, C. and {Nichol}, R.~C. and {Wasserman}, L.},
    title = "{A New Source Detection Algorithm Using the False-Discovery Rate}",
  journal = {\aj},
   eprint = {astro-ph/0110570},
 keywords = {Methods: Data Analysis, Methods: Statistical, Techniques: Image Processing},
     year = 2002,
    month = feb,
   volume = 123,
    pages = {1086},
      doi = {10.1086/338316},
   adsurl = {http://adsabs.harvard.edu/abs/2002AJ....123.1086H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{sdssedr,
   author = {{Stoughton}, C. and {Lupton}, R.~H. and {Bernardi}, M. and {Blanton}, M.~R. and
	{Burles}, S. and {Castander}, F.~J. and {Connolly}, A.~J. and
	{Eisenstein}, D.~J. and {Frieman}, J.~A. and {Hennessy}, G.~S. and
	{Hindsley}, R.~B. and {Ivezi{\'c}}, {\v Z}. and {Kent}, S. and
	{Kunszt}, P.~Z. and {Lee}, B.~C. and {Meiksin}, A. and {Munn}, J.~A. and
	{Newberg}, H.~J. and {Nichol}, R.~C. and {Nicinski}, T. and
	{Pier}, J.~R. and {Richards}, G.~T. and {Richmond}, M.~W. and
	{Schlegel}, D.~J. and {Smith}, J.~A. and {Strauss}, M.~A. and
	{SubbaRao}, M. and {Szalay}, A.~S. and {Thakar}, A.~R. and {Tucker}, D.~L. and
	{Vanden Berk}, D.~E. and {Yanny}, B. and {Adelman}, J.~K. and
	{Anderson}, Jr., J.~E. and {Anderson}, S.~F. and {Annis}, J. and
	{Bahcall}, N.~A. and {Bakken}, J.~A. and {Bartelmann}, M. and
	{Bastian}, S. and {Bauer}, A. and {Berman}, E. and {B{\"o}hringer}, H. and
	{Boroski}, W.~N. and {Bracker}, S. and {Briegel}, C. and {Briggs}, J.~W. and
	{Brinkmann}, J. and {Brunner}, R. and {Carey}, L. and {Carr}, M.~A. and
	{Chen}, B. and {Christian}, D. and {Colestock}, P.~L. and {Crocker}, J.~H. and
	{Csabai}, I. and {Czarapata}, P.~C. and {Dalcanton}, J. and
	{Davidsen}, A.~F. and {Davis}, J.~E. and {Dehnen}, W. and {Dodelson}, S. and
	{Doi}, M. and {Dombeck}, T. and {Donahue}, M. and {Ellman}, N. and
	{Elms}, B.~R. and {Evans}, M.~L. and {Eyer}, L. and {Fan}, X. and
	{Federwitz}, G.~R. and {Friedman}, S. and {Fukugita}, M. and
	{Gal}, R. and {Gillespie}, B. and {Glazebrook}, K. and {Gray}, J. and
	{Grebel}, E.~K. and {Greenawalt}, B. and {Greene}, G. and {Gunn}, J.~E. and
	{de Haas}, E. and {Haiman}, Z. and {Haldeman}, M. and {Hall}, P.~B. and
	{Hamabe}, M. and {Hansen}, B. and {Harris}, F.~H. and {Harris}, H. and
	{Harvanek}, M. and {Hawley}, S.~L. and {Hayes}, J.~J.~E. and
	{Heckman}, T.~M. and {Helmi}, A. and {Henden}, A. and {Hogan}, C.~J. and
	{Hogg}, D.~W. and {Holmgren}, D.~J. and {Holtzman}, J. and {Huang}, C.-H. and
	{Hull}, C. and {Ichikawa}, S.-I. and {Ichikawa}, T. and {Johnston}, D.~E. and
	{Kauffmann}, G. and {Kim}, R.~S.~J. and {Kimball}, T. and {Kinney}, E. and
	{Klaene}, M. and {Kleinman}, S.~J. and {Klypin}, A. and {Knapp}, G.~R. and
	{Korienek}, J. and {Krolik}, J. and {Kron}, R.~G. and {Krzesi{\'n}ski}, J. and
	{Lamb}, D.~Q. and {Leger}, R.~F. and {Limmongkol}, S. and {Lindenmeyer}, C. and
	{Long}, D.~C. and {Loomis}, C. and {Loveday}, J. and {MacKinnon}, B. and
	{Mannery}, E.~J. and {Mantsch}, P.~M. and {Margon}, B. and {McGehee}, P. and
	{McKay}, T.~A. and {McLean}, B. and {Menou}, K. and {Merelli}, A. and
	{Mo}, H.~J. and {Monet}, D.~G. and {Nakamura}, O. and {Narayanan}, V.~K. and
	{Nash}, T. and {Neilsen}, Jr., E.~H. and {Newman}, P.~R. and
	{Nitta}, A. and {Odenkirchen}, M. and {Okada}, N. and {Okamura}, S. and
	{Ostriker}, J.~P. and {Owen}, R. and {Pauls}, A.~G. and {Peoples}, J. and
	{Peterson}, R.~S. and {Petravick}, D. and {Pope}, A. and {Pordes}, R. and
	{Postman}, M. and {Prosapio}, A. and {Quinn}, T.~R. and {Rechenmacher}, R. and
	{Rivetta}, C.~H. and {Rix}, H.-W. and {Rockosi}, C.~M. and {Rosner}, R. and
	{Ruthmansdorfer}, K. and {Sandford}, D. and {Schneider}, D.~P. and
	{Scranton}, R. and {Sekiguchi}, M. and {Sergey}, G. and {Sheth}, R. and
	{Shimasaku}, K. and {Smee}, S. and {Snedden}, S.~A. and {Stebbins}, A. and
	{Stubbs}, C. and {Szapudi}, I. and {Szkody}, P. and {Szokoly}, G.~P. and
	{Tabachnik}, S. and {Tsvetanov}, Z. and {Uomoto}, A. and {Vogeley}, M.~S. and
	{Voges}, W. and {Waddell}, P. and {Walterbos}, R. and {Wang}, S.-i. and
	{Watanabe}, M. and {Weinberg}, D.~H. and {White}, R.~L. and
	{White}, S.~D.~M. and {Wilhite}, B. and {Wolfe}, D. and {Yasuda}, N. and
	{York}, D.~G. and {Zehavi}, I. and {Zheng}, W.},
    title = "{Sloan Digital Sky Survey: Early Data Release}",
  journal = {\aj},
 keywords = {Atlases, Catalogs, Surveys},
     year = 2002,
    month = jan,
   volume = 123,
    pages = {485},
      doi = {10.1086/324741},
   adsurl = {http://adsabs.harvard.edu/abs/2002AJ....123..485S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{miller01,
   author = {{Miller}, C.~J. and {Genovese}, C. and {Nichol}, R.~C. and {Wasserman}, L. and
	{Connolly}, A. and {Reichart}, D. and {Hopkins}, A. and {Schneider}, J. and
	{Moore}, A.},
    title = "{Controlling the False-Discovery Rate in Astrophysical Data Analysis}",
  journal = {\aj},
   eprint = {astro-ph/0107034},
 keywords = {Methods: Analytical, Methods: Data Analysis, Methods: Statistical, Techniques: Image Processing},
     year = 2001,
    month = dec,
   volume = 122,
    pages = {3492},
      doi = {10.1086/324109},
   adsurl = {http://adsabs.harvard.edu/abs/2001AJ....122.3492M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{vDcosmicrays,
   author = {{van Dokkum}, P.~G.},
    title = "{Cosmic-Ray Rejection by Laplacian Edge Detection}",
  journal = {\pasp},
   eprint = {astro-ph/0108003},
 keywords = {Instrumentation: Detectors, Methods: Data Analysis-techniques: image processing},
     year = 2001,
    month = nov,
   volume = 113,
    pages = {1420},
      doi = {10.1086/323894},
   adsurl = {http://adsabs.harvard.edu/abs/2001PASP..113.1420V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{laferte2000,
   author = {{Laferte}, J.-M. and {Perez}, P. and {Heitz}, F.},
    title = "{Discrete Markov image modeling and inference on the quadtree}",
  journal = {ITIP},
     year = 2000,
    month = mar,
   volume = 9,
    pages = {390},
      doi = {10.1109/83.826777},
   adsurl = {http://adsabs.harvard.edu/abs/2000ITIP....9..390L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{degrijs2001,
   author = {{de Grijs}, R. and {Kregel}, M. and {Wesson}, K.~H.},
    title = "{Radially truncated galactic discs}",
  journal = {\mnras},
   eprint = {astro-ph/0002523},
 keywords = {GALAXIES: FORMATION, GALAXIES: FUNDAMENTAL PARAMETERS, GALAXIES: PHOTOMETRY, GALAXIES: SPIRAL, GALAXIES: STRUCTURE},
     year = 2001,
    month = jul,
   volume = 324,
    pages = {1074},
      doi = {10.1046/j.1365-8711.2001.04380.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.324.1074D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{lupton99,
   author = {{Lupton}, R.~H. and {Gunn}, J.~E. and {Szalay}, A.~S.},
    title = "{A Modified Magnitude System that Produces Well-Behaved Magnitudes, Colors, and Errors Even for Low Signal-to-Noise Ratio Measurements}",
  journal = {\aj},
   eprint = {astro-ph/9903081},
 keywords = {CATALOGS, METHODS: STATISTICAL, TECHNIQUES: PHOTOMETRIC},
     year = 1999,
    month = sep,
   volume = 118,
    pages = {1406},
      doi = {10.1086/301004},
   adsurl = {http://adsabs.harvard.edu/abs/1999AJ....118.1406L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{klypin1999,
   author = {{Klypin}, A. and {Kravtsov}, A.~V. and {Valenzuela}, O. and
	{Prada}, F.},
    title = "{Where Are the Missing Galactic Satellites?}",
  journal = {\apj},
   eprint = {astro-ph/9901240},
 keywords = {COSMOLOGY: THEORY, GALAXIES: CLUSTERS: GENERAL, GALAXIES: INTERACTIONS, GALAXY: FORMATION, GALAXIES: LOCAL GROUP, METHODS: NUMERICAL, Cosmology: Theory, Galaxies: Clusters: General, Galaxies: Interactions, Galaxy: Formation, Galaxies: Local Group, Methods: Numerical},
     year = 1999,
    month = sep,
   volume = 522,
    pages = {82},
      doi = {10.1086/307643},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...522...82K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@article{fftw,
 author = {Frigo, Matteo},
 title = {A Fast Fourier Transform Compiler},
 journal = {SIGPLAN Not.},
 issue_date = {May 1999},
 volume = {34},
 number = {5},
 month = may,
 year = {1999},
 issn = {0362-1340},
 pages = {169},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/301631.301661},
 doi = {10.1145/301631.301661},
 acmid = {301661},
 publisher = {ACM},
 address = {New York, NY, USA},
}






@ARTICLE{vdBergh96,
   author = {{van den Bergh}, S. and {Abraham}, R.~G. and {Ellis}, R.~S. and
	{Tanvir}, N.~R. and {Santiago}, B.~X. and {Glazebrook}, K.~G.
	},
    title = "{A Morphological Catalog of Galaxies in the Hubble deep Field}",
  journal = {\aj},
   eprint = {astro-ph/9604161},
 keywords = {CATALOGS, GALAXIES: FUNDAMENTAL PARAMETERS},
     year = 1996,
    month = aug,
   volume = 112,
    pages = {359},
      doi = {10.1086/118020},
   adsurl = {http://adsabs.harvard.edu/abs/1996AJ....112..359V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{sextractor,
   author = {{Bertin}, E. and {Arnouts}, S.},
    title = "{SExtractor: Software for source extraction.}",
  journal = {\aaps},
 keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
     year = 1996,
    month = jun,
   volume = 117,
    pages = {393},
      doi = {10.1051/aas:1996164},
   adsurl = {http://ads.nao.ac.jp/abs/1996A&AS..117..393B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{abraham96,
   author = {{Abraham}, R.~G. and {van den Bergh}, S. and {Glazebrook}, K. and
	{Ellis}, R.~S. and {Santiago}, B.~X. and {Surma}, P. and {Griffiths}, R.~E.
	},
    title = "{The Morphologies of Distant Galaxies. II. Classifications from the Hubble Space Telescope Medium Deep Survey}",
  journal = {\apjs},
 keywords = {GALAXIES: EVOLUTION, GALAXIES: FUNDAMENTAL PARAMETERS, GALAXIES: INTERACTIONS, SURVEYS},
     year = 1996,
    month = nov,
   volume = 107,
    pages = {1},
      doi = {10.1086/192352},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJS..107....1A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{cowie95,
   author = {{Cowie}, L.~L. and {Hu}, E.~M. and {Songaila}, A.},
    title = "{Faintest Galaxy Morphologies From HST WFPC2 Imaging of the Hawaii Survey Fields}",
  journal = {\aj},
   eprint = {astro-ph/9507055},
 keywords = {GALAXIES: EVOLUTION, GALAXIES: FUNDAMENTAL PARAMETERS},
     year = 1995,
    month = oct,
   volume = 110,
    pages = {1576},
      doi = {10.1086/117631},
   adsurl = {http://adsabs.harvard.edu/abs/1995AJ....110.1576C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{williams94,
   author = {{Williams}, J.~P. and {de Geus}, E.~J. and {Blitz}, L.},
    title = "{Determining structure in molecular clouds}",
  journal = {\apj},
 keywords = {Evolution (Development), Mass Spectra, Molecular Clouds, Size (Dimensions), Spectral Line Width, Star Formation, Stellar Structure, Temperature, Algorithms, Least Squares Method, Line Spectra, Mapping, Numerical Analysis, Simulation},
     year = 1994,
    month = jun,
   volume = 428,
    pages = {693},
      doi = {10.1086/174279},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...428..693W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Kauffmann93,
   author = {{Kauffmann}, G. and {White}, S.~D.~M. and {Guiderdoni}, B.},
    title = "{The Formation and Evolution of Galaxies Within Merging Dark Matter Haloes}",
  journal = {\mnras},
     year = 1993,
    month = sep,
   volume = 264,
    pages = {201},
   adsurl = {http://adsabs.harvard.edu/abs/1993MNRAS.264..201K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@book{dougherty92,
 author    = "{Dougherty}, E.",
 title     = "Mathematical Morphology in Image Processing",
 publisher = "CRC Press",
 year      =  1992,
 edition   = "1st",
 isbn      = "9780824787240"
}






@ARTICLE{vcwatershed,
   author = {Vincent, L. and Soille, P.},
  journal = {ITPAM},
    title = {Watersheds in digital spaces: an efficient algorithm based on immersion simulations},
     year = {1991},
    month = {Jun},
   volume = {13},
   number = {6},
    pages = {583},
 keywords = {computerised picture processing;computerised picture processing;digital elevation models;digital gray-scale images;magnetic resonance imagery;picture segmentation;pseudo C language;watersheds;Computational modeling;Digital elevation models;Digital images;Floods;Gray-scale;Image processing;Image segmentation;Morphology;Oceans;Surfaces},
      doi = {10.1109/34.87344},
     ISSN = {0162-8828},
}





@ARTICLE{beard90,
   author = {{Beard}, S.~M. and {MacGillivray}, H.~T. and {Thanisch}, P.~F.
	},
    title = "{The Cosmos System for Crowded-Field Analysis of Digitized Photographic Plate Scans}",
  journal = {\mnras},
     year = 1990,
    month = nov,
   volume = 247,
    pages = {311},
   adsurl = {http://adsabs.harvard.edu/abs/1990MNRAS.247..311B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{kennicutt89,
   author = {{Kennicutt}, Jr., R.~C.},
    title = "{The star formation law in galactic disks}",
  journal = {\apj},
 keywords = {Galactic Evolution, H Alpha Line, H Ii Regions, Interstellar Gas, Star Formation Rate, Emission Spectra, Gas Dynamics, Radial Distribution, Spiral Galaxies},
     year = 1989,
    month = sep,
   volume = 344,
    pages = {685},
      doi = {10.1086/167834},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...344..685K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{infante87,
   author = {{Infante}, L.},
    title = "{A faint object processing software - Description and testing}",
  journal = {\aap},
 keywords = {Astronomical Photography, Computer Programs, Computerized Simulation, Faint Objects, Image Processing, Algorithms, Astronomical Photometry, Galaxies, Red Shift, Stars},
     year = 1987,
    month = sep,
   volume = 183,
    pages = {177},
   adsurl = {http://adsabs.harvard.edu/abs/1987A&A...183..177I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{daophot,
   author = {{Stetson}, P.~B.},
    title = "{DAOPHOT - A computer program for crowded-field stellar photometry}",
  journal = {\pasp},
 keywords = {Algorithms, Astronomical Photometry, Computer Programs, Charge Coupled Devices, Color-Magnitude Diagram, Magellanic Clouds, Point Spread Functions, Television Cameras},
     year = 1987,
    month = mar,
   volume = 99,
    pages = {191},
      doi = {10.1086/131977},
   adsurl = {http://adsabs.harvard.edu/abs/1987PASP...99..191S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{lupton86,
   author = {{Lupton}, R.~H. and {Gunn}, J.~E.},
    title = "{M13 - Main sequence photometry and the mass function}",
  journal = {\aj},
 keywords = {Astronomical Photometry, Main Sequence Stars, Mass Ratios, Stellar Mass, Accuracy, Data Reduction, Stellar Color, Stellar Luminosity, Stellar Magnitude},
     year = 1986,
    month = feb,
   volume = 91,
    pages = {317},
      doi = {10.1086/114012},
   adsurl = {http://adsabs.harvard.edu/abs/1986AJ.....91..317L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{irwin85,
   author = {{Irwin}, M.~J.},
    title = "{Automatic analysis of crowded fields}",
  journal = {\mnras},
 keywords = {Astronomical Photometry, Automation, Background Radiation, Image Analysis, Parameter Identification, Computer Techniques, Data Reduction, Globular Clusters, Maximum Likelihood Estimates, Signal Detection, Sky Radiation},
     year = 1985,
    month = jun,
   volume = 214,
    pages = {575},
   adsurl = {http://adsabs.harvard.edu/abs/1985MNRAS.214..575I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{ratnatunga84,
   author = {{Ratnatunga}, K.~U. and {Newell}, E.~B.},
    title = "{The reduction of panoramic photometry. III - an asymmetric clipping algorithm}",
  journal = {\aj},
 keywords = {Astronomical Photometry, Data Reduction, Image Processing, Algorithms, Galactic Nuclei, Galaxies, Photographic Plates},
     year = 1984,
    month = jan,
   volume = 89,
    pages = {176},
      doi = {10.1086/113498},
   adsurl = {http://adsabs.harvard.edu/abs/1984AJ.....89..176R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{kron,
   author = {{Kron}, R.~G.},
    title = "{Photometry of a complete sample of faint galaxies}",
  journal = {\apjs},
 keywords = {ASTRONOMICAL PHOTOMETRY, GALACTIC RADIATION, GALAXIES, STAR DISTRIBUTION, CALIBRATING, COLORIMETRY, DISTRIBUTION FUNCTIONS, GALACTIC EVOLUTION, LUMINOUS INTENSITY, TABLES (DATA)},
     year = 1980,
    month = jun,
   volume = 43,
    pages = {305},
      doi = {10.1086/190669},
   adsurl = {http://adsabs.harvard.edu/abs/1980ApJS...43..305K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@book{hawkins80,
    author    = "{Hawkins}, D. M.",
    title     = "Identification of outliers",
    publisher = "Chapman \& Hall",
    year      = "1980",
    isbn      = "978-94-015-3996-8"
}




@ARTICLE{bijaoui80,
   author = {{Bijaoui}, A.},
    title = "{Sky background estimation and application}",
  journal = {\aap},
 keywords = {Astronomical Photography, Background Radiation, Computer Techniques, Photographic Plates, Astronomical Maps, Histograms, Image Processing, Planetary Nebulae},
     year = 1980,
    month = apr,
   volume = 84,
    pages = {81},
   adsurl = {http://adsabs.harvard.edu/abs/1980A&A....84...81B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{petrosian,
   author = {{Petrosian}, V.},
    title = "{Surface brightness and evolution of galaxies}",
  journal = {\apjl},
 keywords = {Astronomical Models, Galactic Evolution, Luminous Intensity, Red Shift, Surface Properties, Big Bang Cosmology, Cosmology, Hubble Diagram, Iterative Solution, Point Sources},
     year = 1976,
    month = oct,
   volume = 209,
    pages = {L1},
      doi = {10.1086/182253},
   adsurl = {http://adsabs.harvard.edu/abs/1976ApJ...209L...1P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@article{anscombe,
   author = {Anscombe, F. J.},
    title = {Graphs in Statistical Analysis},
  journal = {The American Statistician},
   volume = {27},
   number = {1},
    pages = {17},
      url = {http://www.jstor.org/stable/2682899},
      doi = {10.2307/2682899},
     ISSN = {00031305},
     year = {1973},
    month = feb,
publisher = {American Statistical Association},
}





@ARTICLE{bijaoui70,
   author = {{Bijaoui}, A. and {Dantel}, M.},
    title = "{Shut's Method}",
  journal = {\aap},
     year = 1970,
    month = may,
   volume = 6,
    pages = {51},
   adsurl = {http://adsabs.harvard.edu/abs/1970A&A.....6...51B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{sersic,
   author = {{S{\'e}rsic}, J.~L.},
    title = "{Influence of the atmospheric and instrumental dispersion on the brightness distribution in a galaxy}",
  journal = {BAAA},
     year = 1963,
   volume = 6,
    pages = {41},
   adsurl = {http://adsabs.harvard.edu/abs/1963BAAA....6...41S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{deVaucClassification,
   author = {{de Vaucouleurs}, G.},
    title = "{Classification and Morphology of External Galaxies.}",
  journal = {Handbuch der Physik},
     year = 1959,
   volume = 53,
    pages = {275},
   adsurl = {http://adsabs.harvard.edu/abs/1959HDP....53..275D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@article {GoldenSection,
    AUTHOR = {Kiefer, J.},
     TITLE = {Sequential minimax search for a maximum},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {4},
      YEAR = {1953},
     PAGES = {502},
      ISSN = {0002-9939},
   MRCLASS = {62.0X},
  MRNUMBER = {0055639 (14,1103h)},
MRREVIEWER = {J. L. Snell},
       doi = {10.1090/S0002-9939-1953-0055639-3},
}






@ARTICLE{hubblefork,
   author = {{Hubble}, E.},
    title = "{No. 324. Extra-galactic nebulae.}",
  journal = {Contributions from the Mount Wilson Observatory / Carnegie Institution of Washington},
     year = 1926,
   volume = 324,
    pages = {1},
   adsurl = {http://adsabs.harvard.edu/abs/1926CMWCI.324....1H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

